Single Fluid vs. Multifluid: Comparison between single fluid and multifluid dust models for disc planet interactions

Recent observations of substructures such as dust gaps and dust rings in protoplanetary discs have highlighted the importance of including dust into purely gaseous disc models. At the same time, computational difficulties arise with the standard models of simulating the dust and gas separately. These include the cost of accurately simulating the interactions between well coupled dust and gas and issues of dust concentration in areas below resolution of the gas phase. We test a single fluid approach, that incorporates the terminal velocity approximation valid for small particles, which can overcome these difficulties, through modification of FARGO3D. We compare this single fluid model with a multifluid model for a variety of planet masses. We find differences in the dust density distribution in all cases. For high-mass, gap-opening planets we find differences in the amplitude of the resulting dust rings, which we attribute to the failure of the terminal velocity approximation around shocks. For low-mass planets, both models agree everywhere except in the corotation region, where the terminal velocity approximation shows overdense dust lobes. We tentatively interpret these as dusty equivalents of thermal lobes seen in non-isothermal simulations with thermal diffusion, but more work is necessary to confirm this. At the same resolution, the computational time for the terminal velocity approximation model is significantly less than a two fluid model. We conclude that the terminal velocity approximation is a valuable tool for modelling a protoplanetary disc but that care should be taken when shocks are involved.

==> scrap.tex <==
{Two Fluid}
    \begin{tabular}{lllll} \toprule
St    & $t_1$  & $t_2$  & $t_3$  & Average Time  \\ \hline
$10^{-1}$ & 86m 52.989s & 87m 40.761s & 87m 47.382s & 87m 27.044s \\ 
$10^{-2}$ & 86m 55.732s & 88m 16.233s & 87m 20.452s & 87m 30.806s \\ 
$10^{-3}$ & 83m 47.744s & 84m 43.551s & 84m 44.812s & 84m 25.369s \\ 
$10^{-4}$ & 83m 30.831s & 84m 2.866s & 84m 51.419s & 84m 8.372s \\ 
$10^{-6}$ & 87m 35.436s & 87m 44.764s & 87m 47.720s & 87m 42.640s \\  \bottomrule
\end{tabular}

{\secondmods 
When the disc aspect ratio is unchanged from $[0.01,0.1]$ but a Neptune planet mass is embedded, corresponding to $100$ and $0.1 M_{th}$ we find that for a lower disc aspect ratio, the Neptune sized planet carves out a gap where the evolution of the dust breaks down with the dust density dropping below zero creating a larger discrepancy between the two models than the disc aspect ratio of 0.05 case. For the higher disc aspect ratio the LITVA model agrees closely with the Two Fluid model in all regions apart from the corotation region behind the planet as a shallow cavity is created in the middle of the asymmetric horseshoe leg. This contrasts to the results in Fig. \ref{fig:neptunecomb} with a disc aspect ratio of $0.05$, corresponding to a planet mass of $0.8 M_{th}$ where the LITVA model did not agree well with the Two Fluid model.

We then ran simulations with a Neptune mass planet with disc aspect ratios of $H/r \in [0.03218... , 0.3218...]$ for 200 orbits to obtain a planet mass of $3$ and $3\times10^{-3} M_{th}$ respectively to see if the LITVA model produced the same agreements and disagreements with the Two Fluid model as the Earth mass planet embedded disc with the same thermal mass. We find that with the lower disc aspect ratio, the results start to diverge from the Two Fluid model with a dust enhancement interior to the planet and gaps near the planet with the dust density dropping below zero. The higher aspect ratio simulations resulted in the two models agreeing closely in all regions apart from one cell width from the radial boundaries. In the one cell width from the inner and outer boundary, the dust density percentage difference was larger than $\pm5\%$ between the two models and everywhere else never exceeded $+0.65\%$ and $-0.23\%$.

With these results and previous ones in subsection \ref{large}, we show that increasing the planet mass while keeping the disc aspect ratio constant leads to disagreements between the two models as does keeping the planet mass constant and decreasing the disc aspect ratio. Therefore it would seem that the thermal mass can play an important role in how well the LITVA model agrees with Two Fluid since keeping the same thermal mass for a different planet mass and disc aspect ratio produces the same comparison between the two models.

}
